A Prognostic, One-Equation Model of Meso-Scale Eddy Momentum Fluxes

We present a prognostic, one-equation model for eddy-mean flow interactions to parameterize the divergence of the Eliassen-Palm flux tensor (EPFT) that arises from thickness-weighted averaging (TWA) the hydrostatic Boussinesq equations. The TWA system of equations does not invoke approximations beyond those for which the hydrostatic Boussinesq equations are valid, constituting a mathematically consistent framework with clear physical interpretations. This model is intended for the adiabatic interior of zonally symmetric flows, in the absence of topographic features, where terms corresponding to eddy interfacial form drag in the EPFT dominate forces. We model eddy interfacial form drag terms for vertical flux of horizontal momentum using the gradient hypothesis, as the product of an eddy viscosity and the vertical gradient of horizontal momentum. We use mixing length theory to relate viscosity to an eddy length scale and an eddy velocity, which is proportional to the eddy energy in the TWA system. The eddy length scale is modeled as the first Rossby radius of deformation, which we calculate as a function of the mean flow. We use a prognostic equation for vertically integrated eddy energy at each horizontal location, which we derive from the TWA framework, and then simplify to the flows of interest by ignoring transport, redistribution and diabatic terms. The prognostic vertically integrated eddy energy is projected onto the water column using the eigenvalue of the first baroclinic mode to obtain the eddy energy at each vertical position. The eddy viscosity has horizontal as well as vertical structure. We diagnosed the model equations in an eddy resolving numerical simulation of a zonally re-entrant channel representative of the Southern Ocean. We have implemented the model parameterization in an ocean model and tested it to simulate a parameterized simulation of this flow.

==> mep_epft.bib-save-2017.12.18_10.25.30 <==


@article{gent_mcwilliams_1990,
  author =        {Gent, Peter R. and McWilliams, James C.},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2012/07/19},
  number =        {1},
  pages =         {150--155},
  publisher =     {American Meteorological Society},
  title =         {Isopycnal Mixing in Ocean Circulation Models},
  volume =        {20},
  year =          {1990},
  annote =        {doi: 10.1175/1520-0485(1990)020<0150:IMIOCM>2.0.CO;2},
  doi =           {10.1175/1520-0485(1990)020<0150:IMIOCM>2.0.CO;2},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/1520-0485(1990)020<0150:
                  IMIOCM>2.0.CO;2},
}

@article{deszoeke_bennett_1993,
  author =        {de Szoeke, Roland A. and Bennett, Andrew F.},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2014/02/14},
  number =        {10},
  pages =         {2254--2264},
  publisher =     {American Meteorological Society},
  title =         {Microstructure Fluxes across Density Surfaces},
  volume =        {23},
  year =          {1993},
  annote =        {doi: 10.1175/1520-0485(1993)023<2254:MFADS>2.0.CO;2},
  doi =           {10.1175/1520-0485(1993)023<2254:MFADS>2.0.CO;2},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/1520-0485(1993)023<2254:
                  MFADS>2.0.CO;2},
}

@article{young_2012,
  author =        {Young, William R.},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2013/06/12},
  number =        {5},
  pages =         {692--707},
  publisher =     {American Meteorological Society},
  title =         {An Exact Thickness-Weighted Average Formulation of
                   the Boussinesq Equations},
  volume =        {42},
  year =          {2012},
  annote =        {doi: 10.1175/JPO-D-11-0102.1},
  doi =           {10.1175/JPO-D-11-0102.1},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/JPO-D-11-0102.1},
}

@article{maddison_marshall_2013,
  author =        {Maddison, J. R. and Marshall, D. P.},
  journal =       {Journal of Fluid Mechanics},
  month =         {8},
  pages =         {69--102},
  title =         {The Eliassen--Palm flux tensor},
  volume =        {729},
  year =          {2013},
  doi =           {10.1017/jfm.2013.259},
  issn =          {1469-7645},
}

@article{visbeck_etal_97,
  author =        {Visbeck, Martin and Marshall, John and Haine, Tom and
                   Spall, Mike},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2013/10/31},
  number =        {3},
  pages =         {381--402},
  publisher =     {American Meteorological Society},
  title =         {Specification of Eddy Transfer Coefficients in
                   Coarse-Resolution Ocean Circulation Models*},
  volume =        {27},
  year =          {1997},
  annote =        {doi: 10.1175/1520-0485(1997)027<0381:SOETCI>2.0.CO;2},
  doi =           {10.1175/1520-0485(1997)027<0381:SOETCI>2.0.CO;2},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/1520-0485(1997)027<0381:
                  SOETCI>2.0.CO;2},
}

@article{ferreira_marshall_2006,
  author =        {D. Ferreira and J. Marshall},
  journal =       {Ocean Modelling},
  number =        {1},
  pages =         {86 - 107},
  title =         {Formulation and implementation of a ``residual-mean''
                   ocean circulation model},
  volume =        {13},
  year =          {2006},
  abstract =      {A parameterization of mesoscale eddies in
                   coarse-resolution ocean general circulation models
                   (GCM) is formulated and implemented using a
                   residual-mean formalism. In that framework, mean
                   buoyancy is advected by the residual velocity (the
                   sum of the Eulerian and eddy-induced velocities) and
                   modified by a residual flux which accounts for the
                   diabatic effects of mesoscale eddies. The residual
                   velocity is obtained by stepping forward a
                   residual-mean momentum equation in which eddy
                   stresses appear as forcing terms. Study of the
                   spatial distribution of eddy stresses, derived by
                   using them as control parameters to ``fit'' the
                   residual-mean model to observations, supports the
                   idea that eddy stresses can be likened to a vertical
                   down-gradient flux of momentum with a coefficient
                   which is constant in the vertical. The residual eddy
                   flux is set to zero in the ocean interior, where
                   mesoscale eddies are assumed to be quasi-adiabatic,
                   but is parameterized by a horizontal down-gradient
                   diffusivity near the surface where eddies develop a
                   diabatic component as they stir properties
                   horizontally across steep isopycnals. The
                   residual-mean model is implemented and tested in the
                   \{MIT\} general circulation model. It is shown that
                   the resulting model (1) has a climatology that is
                   superior to that obtained using the Gent and
                   McWilliams parameterization scheme with a spatially
                   uniform diffusivity and (2) allows one to
                   significantly reduce the (spurious) horizontal
                   viscosity used in coarse-resolution GCMs.},
  doi =           {http://dx.doi.org/10.1016/j.ocemod.2005.12.001},
  issn =          {1463-5003},
  url =           {http://www.sciencedirect.com/science/article/pii/
                  S1463500305001022},
}

@article{eden_greatbatch_2008,
  author =        {Carsten Eden and Richard J. Greatbatch},
  journal =       {Ocean Modelling},
  number =        {3},
  pages =         {223 - 239},
  title =         {Towards a mesoscale eddy closure},
  volume =        {20},
  year =          {2008},
  doi =           {http://dx.doi.org/10.1016/j.ocemod.2007.09.002},
  issn =          {1463-5003},
  url =           {http://www.sciencedirect.com/science/article/pii/
                  S1463500307001163},
}

@article{saenz_etal_2015a,
  author =        {Saenz, Juan A. and Chen, Qingshan and Ringler, Todd},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2015/07/24},
  publisher =     {American Meteorological Society},
  title =         {Prognostic residual-mean flow in an ocean general
                   circulation model and its relation to prognostic
                   Eulerian-mean flow},
  year =          {2015},
  abstract =      {AbstractRecent work has shown that thickness-weighted
                   averaging (TWA) the Boussinesq equations in buoyancy
                   coordinates results in exact equations governing the
                   prognostic residual-mean flow where eddy-mean flow
                   interactions appear in the horizontal momentum
                   equations as the divergence of the Eliassen-Palm Flux
                   tensor (EPFT). It has been proposed that, given the
                   mathematical tractability of the TWA equations, the
                   physical interpretation of the EPFT and its relation
                   to potential vorticity fluxes, the TWA is an
                   appropriate framework for modeling ocean circulation
                   with parameterized eddies. We test the feasibility of
                   this proposition and investigate the connections
                   between the TWA framework and the conventional
                   framework used in models, where Eulerian-mean flow
                   prognostic variables are solved for. Using the TWA
                   framework as a starting point, we explore the well
                   known connections between vertical transfer of
                   horizontal momentum by eddy form drag and eddy
                   overturning by the bolus velocity, used by Greatbatch
                   and Lamb (1990) and Gent and McWilliams (1990) (GM)
                   to parameterize eddies. After implementing the TWA
                   framework in an ocean general circulation model, we
                   verify our analysis by comparing the flows in an
                   idealized Southern Ocean configuration simulated
                   using the TWA and conventional frameworks with the
                   same meso-scale eddy parameterization.},
  annote =        {doi: 10.1175/JPO-D-15-0024.1},
  doi =           {10.1175/JPO-D-15-0024.1},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/JPO-D-15-0024.1},
}

@article{greatbatch_lamb_1990,
  author =        {Greatbatch, Richard J. and Lamb, Kevin G.},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2014/10/28},
  number =        {10},
  pages =         {1634--1637},
  publisher =     {American Meteorological Society},
  title =         {On Parameterizing Vertical Mixing of Momentum in
                   Non-eddy Resolving Ocean Models},
  volume =        {20},
  year =          {1990},
  abstract =      {Abstract We investigate the consequence, at small
                   Ekman number, of adding vertical mixing of momentum
                   terms to the incompressible thermocline equations. We
                   find that choosing the vertical eddy viscosity, ? =
                   Af2/N2, where f is the Coriolis parameter and N is
                   the local value of the buoyancy frequency, leads to
                   isopycnal mixing of fQ, where Q is the reciprocal of
                   potential vorticity, provided A is independent of the
                   vertical coordinate. If, additionally, A is also
                   independent of the north?south coordinate, then on a
                   beta-plane, this implies homogenization of potential
                   vorticity, q, within closed q-contours on isopycnal
                   surfaces. This conclusion extends to spherical
                   geometry if ? is also inversely proportional to ?,
                   the gradient of f with respect to latitude, i.e. ? =
                   Af2/(N2?). The connection with the recent work of
                   Gent and McWilliams and the consequences for coarse
                   resolution numerical model studies are discussed.},
  annote =        {doi: 10.1175/1520-0485(1990)020<1634:OPVMOM>2.0.CO;2},
  doi =           {10.1175/1520-0485(1990)020<1634:OPVMOM>2.0.CO;2},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/1520-0485(1990)020<1634:
                  OPVMOM>2.0.CO;2},
}

@article{ferrari_nikurashin_2010,
  author =        {Ferrari, Raffaele and Nikurashin, Maxim},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2015/03/11},
  number =        {7},
  pages =         {1501--1519},
  publisher =     {American Meteorological Society},
  title =         {Suppression of Eddy Diffusivity across Jets in the
                   Southern Ocean},
  volume =        {40},
  year =          {2010},
  abstract =      {Abstract Geostrophic eddies control the meridional
                   mixing of heat, carbon, and other climatically
                   important tracers in the Southern Ocean. The rate of
                   eddy mixing is typically quantified through an eddy
                   diffusivity. There is an ongoing debate as to whether
                   eddy mixing in enhanced in the core of the Antarctic
                   Circumpolar Current or on its flanks. A simple
                   expression is derived that predicts the rate of eddy
                   mixing, that is, the eddy diffusivity, as a function
                   of eddy and mean current statistics. This novel
                   expression predicts suppression of the cross-jet eddy
                   diffusivity in the core of the Antarctic Circumpolar
                   Current, despite enhanced values of eddy kinetic
                   energy. The expression is qualitatively and
                   quantitatively validated by independent estimates of
                   eddy mixing from altimetry observations. This work
                   suggests that the meridional eddy diffusivity across
                   the Antarctic Circumpolar Current is weaker than
                   presently assumed because of the suppression of eddy
                   mixing by the strong zonal current.},
  annote =        {doi: 10.1175/2010JPO4278.1},
  doi =           {10.1175/2010JPO4278.1},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/2010JPO4278.1},
}

@article{smith_2007,
  author =        {Smith, K. Shafer},
  journal =       {Journal of Marine Research},
  number =        {5},
  pages =         {655-683},
  title =         {The geography of linear baroclinic instability in
                   Earth's oceans},
  volume =        {65},
  year =          {2007},
  doi =           {doi:10.1357/002224007783649484},
}

@article{smith_marshall_2009,
  author =        {Smith, K. Shafer and Marshall, John},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2015/05/27},
  number =        {1},
  pages =         {50--69},
  publisher =     {American Meteorological Society},
  title =         {Evidence for Enhanced Eddy Mixing at Middepth in the
                   Southern Ocean},
  volume =        {39},
  year =          {2009},
  abstract =      {Abstract Satellite altimetric observations of the
                   ocean reveal surface pressure patterns in the core of
                   the Antarctic Circumpolar Current (ACC) that
                   propagate downstream (eastward) but slower than the
                   mean surface current by about 25{\%}. The authors
                   argue that these observations are suggestive of
                   baroclinically unstable waves that have a steering
                   level at a depth of about 1 km. Detailed linear
                   stability calculations using a hydrographic atlas
                   indeed reveal a steering level in the ACC near the
                   depth implied by the altimetric observations.
                   Calculations using a nonlinear model forced by the
                   mean shear and stratification observed close to the
                   core of the ACC, coinciding with a position where
                   mooring data and direct eddy flux measurements are
                   available, reveal a similar picture, albeit with
                   added details. When eddy fluxes are allowed to adjust
                   the mean state, computed eddy kinetic energy and eddy
                   stress are close to observed magnitudes with steering
                   levels between 1 and 1.5 km, broadly consistent with
                   observations. An important result of this study is
                   that the vertical structure of the potential
                   vorticity (PV) eddy diffusivity is strongly depth
                   dependent, implying that the diffusivity for PV and
                   buoyancy are very different from one another. It is
                   shown that the flow can simultaneously support a PV
                   diffusivity peaking at 5000 m2 s?1 or so near the
                   middepth steering level and a buoyancy diffusivity
                   that is much smaller, of order 1000 m2 s?1,
                   exhibiting less vertical structure. An effective
                   diffusivity calculation, using an advected and
                   diffused tracer transformed into area coordinates,
                   confirms that the PV diffusivity more closely
                   reflects the mixing properties of the flow than does
                   the buoyancy diffusivity, and points explicitly to
                   the need for separating tracer and buoyancy flux
                   parameterizations in coarse-resolution general
                   circulation models. Finally, implications for the
                   eddy-driven circulation of the ACC are discussed.},
  annote =        {doi: 10.1175/2008JPO3880.1},
  doi =           {10.1175/2008JPO3880.1},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/2008JPO3880.1},
}

@article{bates_etal_2014,
  author =        {Bates, Michael and Tulloch, Ross and Marshall, John and
                   Ferrari, Raffaele},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2015/03/12},
  number =        {6},
  pages =         {1523--1540},
  publisher =     {American Meteorological Society},
  title =         {Rationalizing the Spatial Distribution of Mesoscale
                   Eddy Diffusivity in Terms of Mixing Length Theory},
  volume =        {44},
  year =          {2014},
  abstract =      {AbstractObservations and theory suggest that lateral
                   mixing by mesoscale ocean eddies only reaches its
                   maximum potential at steering levels, surfaces at
                   which the propagation speed of eddies approaches that
                   of the mean flow. Away from steering levels, mixing
                   is strongly suppressed because the mixing length is
                   smaller than the eddy scale, thus reducing the mixing
                   rates. The suppression is particularly pronounced in
                   strong currents where mesoscale eddies are most
                   energetic. Here, a framework for parameterizing eddy
                   mixing is explored that attempts to capture this
                   suppression. An expression of the surface eddy
                   diffusivity proposed by Ferrari and Nikurashin is
                   evaluated using observations of eddy kinetic energy,
                   eddy scale, and eddy propagation speed. The resulting
                   global maps of eddy diffusivity have a broad
                   correspondence with recent estimates of diffusivity
                   based on the rate at which tracer contours are
                   stretched by altimetric-derived surface currents.
                   Finally, the expression for the eddy diffusivity is
                   extrapolated in the vertical to infer the
                   eddy-induced meridional heat transport and the
                   overturning streamfunction.},
  annote =        {doi: 10.1175/JPO-D-13-0130.1},
  doi =           {10.1175/JPO-D-13-0130.1},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/JPO-D-13-0130.1},
}

@book{smith_book_1997,
  author =        {Smith, Steven W and others},
  editor =        {California Technical Pub. San Diego},
  title =         {The scientist and engineer's guide to digital signal
                   processing},
  year =          {1997},
}

@article{chelton_etal_1998,
  author =        {Chelton, Dudley B. and deSzoeke, Roland A. and
                   Schlax, Michael G. and El Naggar, Karim and
                   Siwertz, Nicolas},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2015/05/27},
  number =        {3},
  pages =         {433--460},
  publisher =     {American Meteorological Society},
  title =         {Geographical Variability of the First Baroclinic
                   Rossby Radius of Deformation},
  volume =        {28},
  year =          {1998},
  abstract =      {Abstract Global 1$\,^{\circ}$?
                   1$\,^{\circ}$climatologies of the first baroclinic
                   gravity-wave phase speed c1 and the Rossby radius of
                   deformation ?1 are computed from climatological
                   average temperature and salinity profiles. These new
                   atlases are compared with previously published
                   5$\,^{\circ}$? 5$\,^{\circ}$coarse resolution maps of
                   ?1 for the Northern Hemisphere and the South Atlantic
                   and with a 1$\,^{\circ}$?
                   1$\,^{\circ}$fine-resolution map of c1 for the
                   tropical Pacific. It is concluded that the methods
                   used in these earlier estimates yield values that are
                   biased systematically low by 5{\%}?15{\%} owing to
                   seemingly minor computational errors. Geographical
                   variations in the new high-resolution maps of c1 and
                   ?1 are discussed in terms of a WKB approximation that
                   elucidates the effects of earth rotation,
                   stratification, and water depth on these quantities.
                   It is shown that the effects of temporal variations
                   of the stratification can be neglected in the
                   estimation of c1 and ?1 at any particular location in
                   the World Ocean. This is rationalized from
                   consideration of the WKB approximation.},
  annote =        {doi: 10.1175/1520-0485(1998)028<0433:GVOTFB>2.0.CO;2},
  doi =           {10.1175/1520-0485(1998)028<0433:GVOTFB>2.0.CO;2},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/1520-0485(1998)028<0433:
                  GVOTFB>2.0.CO;2},
}

@article{ringler_etal_2013,
  author =        {Todd Ringler and Mark Petersen and Robert L. Higdon and
                   Doug Jacobsen and Philip W. Jones and Mathew Maltrud},
  journal =       {Ocean Modelling},
  number =        {0},
  pages =         {211 - 232},
  title =         {A multi-resolution approach to global ocean modeling},
  volume =        {69},
  year =          {2013},
  doi =           {10.1016/j.ocemod.2013.04.010},
  issn =          {1463-5003},
  url =           {http://www.sciencedirect.com/science/article/pii/
                  S1463500313000760},
}

@article{thuburn_etal_2009,
  author =        {J. Thuburn and T.D. Ringler and W.C. Skamarock and
                   J.B. Klemp},
  journal =       {Journal of Computational Physics},
  number =        {22},
  pages =         {8321 - 8335},
  title =         {Numerical representation of geostrophic modes on
                   arbitrarily structured C-grids},
  volume =        {228},
  year =          {2009},
  abstract =      {A C-grid staggering, in which the mass variable is
                   stored at cell centers and the normal velocity
                   component is stored at cell faces (or edges in two
                   dimensions) is attractive for atmospheric modeling
                   since it enables a relatively accurate representation
                   of fast wave modes. However, the discretization of
                   the Coriolis terms is non-trivial. For constant
                   Coriolis parameter, the linearized shallow water
                   equations support geostrophic modes: stationary
                   solutions in geostrophic balance. A naive
                   discretization of the Coriolis terms can cause
                   geostrophic modes to become non-stationary, causing
                   unphysical behaviour of numerical solutions. Recent
                   work has shown how to discretize the Coriolis terms
                   on a planar regular hexagonal grid to ensure that
                   geostrophic modes are stationary while the Coriolis
                   terms remain energy conserving. In this paper this
                   result is extended to arbitrarily structured C-grids.
                   An explicit formula is given for constructing an
                   appropriate discretization of the Coriolis terms. The
                   general formula is illustrated by showing that it
                   recovers previously known results for the planar
                   regular hexagonal C-grid and the spherical
                   longitude--latitude C-grid. Numerical calculation
                   confirms that the scheme does indeed give stationary
                   geostrophic modes for the hexagonal--pentagonal and
                   triangular geodesic C-grids on the sphere.},
  doi =           {http://dx.doi.org/10.1016/j.jcp.2009.08.006},
  issn =          {0021-9991},
  url =           {http://www.sciencedirect.com/science/article/pii/
                  S0021999109004434},
}

@article{ringler_etal_2010,
  author =        {T.D. Ringler and J. Thuburn and J.B. Klemp and
                   W.C. Skamarock},
  journal =       {Journal of Computational Physics},
  number =        {9},
  pages =         {3065 - 3090},
  title =         {A unified approach to energy conservation and
                   potential vorticity dynamics for
                   arbitrarily-structured C-grids},
  volume =        {229},
  year =          {2010},
  doi =           {http://dx.doi.org/10.1016/j.jcp.2009.12.007},
  issn =          {0021-9991},
  url =           {http://www.sciencedirect.com/science/article/pii/
                  S0021999109006780},
}

@article{petersen_etal_2014,
  author =        {Mark R. Petersen and Douglas W. Jacobsen and
                   Todd D. Ringler and Matthew W. Hecht and
                   Mathew E. Maltrud},
  journal =       {Ocean Modelling},
  number =        {0},
  pages =         {93 - 113},
  title =         {Evaluation of the arbitrary Lagrangian--Eulerian
                   vertical coordinate method in the MPAS-Ocean model},
  volume =        {86},
  year =          {2015},
  doi =           {http://dx.doi.org/10.1016/j.ocemod.2014.12.004},
  issn =          {1463-5003},
  url =           {http://www.sciencedirect.com/science/article/pii/
                  S1463500314001796},
}

@article{skamarock_gassmann_2011,
  author =        {Skamarock, William C. and Gassmann, Almut},
  booktitle =     {Monthly Weather Review},
  journal =       {Monthly Weather Review},
  month =         {2014/12/11},
  number =        {9},
  pages =         {2962--2975},
  publisher =     {American Meteorological Society},
  title =         {Conservative Transport Schemes for Spherical Geodesic
                   Grids: High-Order Flux Operators for ODE-Based Time
                   Integration},
  volume =        {139},
  year =          {2011},
  abstract =      {AbstractHigher-order finite-volume flux operators for
                   transport algorithms used within Runge?Kutta time
                   integration schemes on irregular Voronoi (hexagonal)
                   meshes are proposed and tested. These operators are
                   generalizations of third- and fourth-order operators
                   currently used in atmospheric models employing
                   regular, orthogonal rectangular meshes.
                   Two-dimensional least squares fit polynomials are
                   used to evaluate the higher-order spatial derivatives
                   needed to cancel the leading-order truncation error
                   terms of the standard second-order centered
                   formulation. Positive definite or monotonic behavior
                   is achieved by applying an appropriate limiter during
                   the final Runge?Kutta stage within a given time
                   step.The third- and fourth-order formulations are
                   evaluated using standard transport tests on the
                   sphere. The new schemes are more accurate and
                   significantly more efficient than the standard
                   second-order scheme and other schemes in the
                   literature examined by the authors. The third-order
                   formulation is equivalent to the fourth-order
                   formulation plus an additional diffusion term that is
                   proportional to the Courant number. An optimal value
                   for the coefficient scaling this diffusion term is
                   chosen based on qualitative evaluation of the test
                   results. Improvements using the higher-order scheme
                   in place of the traditional second-order centered
                   approach are illustrated within 3D unstable
                   baroclinic wave simulations produced using two global
                   nonhydrostatic models employing spherical Voronoi
                   meshes.},
  annote =        {doi: 10.1175/MWR-D-10-05056.1},
  doi =           {10.1175/MWR-D-10-05056.1},
  isbn =          {0027-0644},
  url =           {http://dx.doi.org/10.1175/MWR-D-10-05056.1},
}

@article{ringler_etal_2017,
  author =        {Todd Ringler and Juan A. Saenz and Phillip J. Wolfram and
                   Luke Van Roekel},
  journal =       {Journal of Physical Oceanography},
  number =        {2},
  pages =         {285-302},
  title =         {A Thickness-Weighted Average Perspective of Force
                   Balance in an Idealized Circumpolar Current},
  volume =        {47},
  year =          {2017},
  abstract =      {AbstractThe exact, three-dimensional,
                   thickness-weighted averaged (TWA) Boussinesq
                   equations are used to diagnose eddy--mean flow
                   interaction in an idealized circumpolar current
                   (ICC). The force exerted by mesoscale eddies on the
                   TWA velocity is expressed as the divergence of the
                   Eliassen--Palm flux tensor. Consistent with previous
                   findings, the analysis indicates that the dynamically
                   relevant definition of the ocean surface layer is
                   composed of the set of buoyancy coordinates that ever
                   reside at the ocean surface at a given horizontal
                   position. The surface layer is found to be a
                   physically distinct object with a diabatic and force
                   balance that is largely isolated from the underlying
                   adiabatic region in the interior. Within the ICC
                   surface layer, the TWA meridional velocity is
                   southward/northward in the top/bottom half and has a
                   value near zero at the bottom. In the top half of the
                   surface layer, the zonal forces due to wind stress
                   and meridional advection of potential vorticity act
                   to accelerate the TWA zonal velocity; equilibrium is
                   obtained by eddies decelerating the zonal flow via a
                   downward flux of eastward momentum that increases
                   with depth. In the bottom half of the surface layer,
                   the accelerating force of the wind stress is balanced
                   by the eddy force and meridional advection of
                   potential vorticity. The bottom of the surface layer
                   coincides with the location where the zonal eddy
                   force, meridional advection of potential vorticity,
                   and zonal wind stress force are all zero. The net
                   meridional transport Sf within the surface layer is a
                   small residual of its southward and northward TWA
                   meridional flows. The mean meridional gradient of the
                   surface layer buoyancy is advected by Sf to balance
                   the surface buoyancy flux.},
  doi =           {10.1175/JPO-D-16-0096.1},
  url =           {http://dx.doi.org/10.1175/JPO-D-16-0096.1},
}

@article{large_etal_1994,
  author =        {Large, W. G. and McWilliams, J. C. and Doney, S. C.},
  journal =       {Rev. Geophys.},
  number =        {4},
  pages =         {363--403},
  publisher =     {AGU},
  title =         {Oceanic vertical mixing: A review and a model with a
                   nonlocal boundary layer parameterization},
  volume =        {32},
  year =          {1994},
  abstract =      {If model parameterizations of unresolved physics,
                   such as the variety of upper ocean mixing processes,
                   are to hold over the large range of time and space
                   scales of importance to climate, they must be
                   strongly physically based. Observations, theories,
                   and models of oceanic vertical mixing are surveyed.
                   Two distinct regimes are identified: ocean mixing in
                   the boundary layer near the surface under a variety
                   of surface forcing conditions (stabilizing,
                   destabilizing, and wind driven), and mixing in the
                   ocean interior due to internal waves, shear
                   instability, and double diffusion (arising from the
                   different molecular diffusion rates of heat and
                   salt). Mixing schemes commonly applied to the upper
                   ocean are shown not to contain some potentially
                   important boundary layer physics. Therefore a new
                   parameterization of oceanic boundary layer mixing is
                   developed to accommodate some of this physics. It
                   includes a scheme for determining the boundary layer
                   depth h, where the turbulent contribution to the
                   vertical shear of a bulk Richardson number is
                   parameterized. Expressions for diffusivity and
                   nonlocal transport throughout the boundary layer are
                   given. The diffusivity is formulated to agree with
                   similarity theory of turbulence in the surface layer
                   and is subject to the conditions that both it and its
                   vertical gradient match the interior values at h.
                   This nonlocal \&{\#}8220;K profile
                   parameterization\&{\#}8221; (KPP) is then verified
                   and compared to alternatives, including its
                   atmospheric counterparts. Its most important feature
                   is shown to be the capability of the boundary layer
                   to penetrate well into a stable thermocline in both
                   convective and wind-driven situations. The
                   diffusivities of the aforementioned three interior
                   mixing processes are modeled as constants, functions
                   of a gradient Richardson number (a measure of the
                   relative importance of stratification to
                   destabilizing shear), and functions of the
                   double-diffusion density ratio, R\&{\#}961;. Oceanic
                   simulations of convective penetration, wind
                   deepening, and diurnal cycling are used to determine
                   appropriate values for various model parameters as
                   weak functions of vertical resolution. Annual cycle
                   simulations at ocean weather station Papa for 1961
                   and 1969\&{\#}8211;1974 are used to test the complete
                   suite of parameterizations. Model and observed
                   temperatures at all depths are shown to agree very
                   well into September, after which systematic advective
                   cooling in the ocean produces expected differences.
                   It is argued that this cooling and a steady salt
                   advection into the model are needed to balance the
                   net annual surface heating and freshwater input. With
                   these advections, good multiyear simulations of
                   temperature and salinity can be achieved. These
                   results and KPP simulations of the diurnal cycle at
                   the Long-Term Upper Ocean Study (LOTUS) site are
                   compared with the results of other models. It is
                   demonstrated that the KPP model exchanges properties
                   between the mixed layer and thermocline in a manner
                   consistent with observations, and at least as well or
                   better than alternatives.},
  isbn =          {8755-1209},
  url =           {http://dx.doi.org/10.1029/94RG01872},
}



==> mep_epft.bib-save-2017.12.22_11.34.37 <==


@article{gent_mcwilliams_1990,
  author =        {Gent, Peter R. and McWilliams, James C.},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2012/07/19},
  number =        {1},
  pages =         {150--155},
  publisher =     {American Meteorological Society},
  title =         {Isopycnal Mixing in Ocean Circulation Models},
  volume =        {20},
  year =          {1990},
  annote =        {doi: 10.1175/1520-0485(1990)020<0150:IMIOCM>2.0.CO;2},
  doi =           {10.1175/1520-0485(1990)020<0150:IMIOCM>2.0.CO;2},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/1520-0485(1990)020<0150:
                  IMIOCM>2.0.CO;2},
}

@article{deszoeke_bennett_1993,
  author =        {de Szoeke, Roland A. and Bennett, Andrew F.},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2014/02/14},
  number =        {10},
  pages =         {2254--2264},
  publisher =     {American Meteorological Society},
  title =         {Microstructure Fluxes across Density Surfaces},
  volume =        {23},
  year =          {1993},
  annote =        {doi: 10.1175/1520-0485(1993)023<2254:MFADS>2.0.CO;2},
  doi =           {10.1175/1520-0485(1993)023<2254:MFADS>2.0.CO;2},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/1520-0485(1993)023<2254:
                  MFADS>2.0.CO;2},
}

@article{young_2012,
  author =        {Young, William R.},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2013/06/12},
  number =        {5},
  pages =         {692--707},
  publisher =     {American Meteorological Society},
  title =         {An Exact Thickness-Weighted Average Formulation of
                   the Boussinesq Equations},
  volume =        {42},
  year =          {2012},
  annote =        {doi: 10.1175/JPO-D-11-0102.1},
  doi =           {10.1175/JPO-D-11-0102.1},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/JPO-D-11-0102.1},
}

@article{maddison_marshall_2013,
  author =        {Maddison, J. R. and Marshall, D. P.},
  journal =       {Journal of Fluid Mechanics},
  month =         {8},
  pages =         {69--102},
  title =         {The Eliassen--Palm flux tensor},
  volume =        {729},
  year =          {2013},
  doi =           {10.1017/jfm.2013.259},
  issn =          {1469-7645},
}

@article{visbeck_etal_97,
  author =        {Visbeck, Martin and Marshall, John and Haine, Tom and
                   Spall, Mike},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2013/10/31},
  number =        {3},
  pages =         {381--402},
  publisher =     {American Meteorological Society},
  title =         {Specification of Eddy Transfer Coefficients in
                   Coarse-Resolution Ocean Circulation Models*},
  volume =        {27},
  year =          {1997},
  annote =        {doi: 10.1175/1520-0485(1997)027<0381:SOETCI>2.0.CO;2},
  doi =           {10.1175/1520-0485(1997)027<0381:SOETCI>2.0.CO;2},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/1520-0485(1997)027<0381:
                  SOETCI>2.0.CO;2},
}

@article{ferreira_marshall_2006,
  author =        {D. Ferreira and J. Marshall},
  journal =       {Ocean Modelling},
  number =        {1},
  pages =         {86 - 107},
  title =         {Formulation and implementation of a ``residual-mean''
                   ocean circulation model},
  volume =        {13},
  year =          {2006},
  abstract =      {A parameterization of mesoscale eddies in
                   coarse-resolution ocean general circulation models
                   (GCM) is formulated and implemented using a
                   residual-mean formalism. In that framework, mean
                   buoyancy is advected by the residual velocity (the
                   sum of the Eulerian and eddy-induced velocities) and
                   modified by a residual flux which accounts for the
                   diabatic effects of mesoscale eddies. The residual
                   velocity is obtained by stepping forward a
                   residual-mean momentum equation in which eddy
                   stresses appear as forcing terms. Study of the
                   spatial distribution of eddy stresses, derived by
                   using them as control parameters to ``fit'' the
                   residual-mean model to observations, supports the
                   idea that eddy stresses can be likened to a vertical
                   down-gradient flux of momentum with a coefficient
                   which is constant in the vertical. The residual eddy
                   flux is set to zero in the ocean interior, where
                   mesoscale eddies are assumed to be quasi-adiabatic,
                   but is parameterized by a horizontal down-gradient
                   diffusivity near the surface where eddies develop a
                   diabatic component as they stir properties
                   horizontally across steep isopycnals. The
                   residual-mean model is implemented and tested in the
                   \{MIT\} general circulation model. It is shown that
                   the resulting model (1) has a climatology that is
                   superior to that obtained using the Gent and
                   McWilliams parameterization scheme with a spatially
                   uniform diffusivity and (2) allows one to
                   significantly reduce the (spurious) horizontal
                   viscosity used in coarse-resolution GCMs.},
  doi =           {http://dx.doi.org/10.1016/j.ocemod.2005.12.001},
  issn =          {1463-5003},
  url =           {http://www.sciencedirect.com/science/article/pii/
                  S1463500305001022},
}

@article{eden_greatbatch_2008,
  author =        {Carsten Eden and Richard J. Greatbatch},
  journal =       {Ocean Modelling},
  number =        {3},
  pages =         {223 - 239},
  title =         {Towards a mesoscale eddy closure},
  volume =        {20},
  year =          {2008},
  doi =           {http://dx.doi.org/10.1016/j.ocemod.2007.09.002},
  issn =          {1463-5003},
  url =           {http://www.sciencedirect.com/science/article/pii/
                  S1463500307001163},
}

@article{saenz_etal_2015a,
  author =        {Saenz, Juan A. and Chen, Qingshan and Ringler, Todd},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2015/07/24},
  publisher =     {American Meteorological Society},
  title =         {Prognostic residual-mean flow in an ocean general
                   circulation model and its relation to prognostic
                   Eulerian-mean flow},
  year =          {2015},
  abstract =      {AbstractRecent work has shown that thickness-weighted
                   averaging (TWA) the Boussinesq equations in buoyancy
                   coordinates results in exact equations governing the
                   prognostic residual-mean flow where eddy-mean flow
                   interactions appear in the horizontal momentum
                   equations as the divergence of the Eliassen-Palm Flux
                   tensor (EPFT). It has been proposed that, given the
                   mathematical tractability of the TWA equations, the
                   physical interpretation of the EPFT and its relation
                   to potential vorticity fluxes, the TWA is an
                   appropriate framework for modeling ocean circulation
                   with parameterized eddies. We test the feasibility of
                   this proposition and investigate the connections
                   between the TWA framework and the conventional
                   framework used in models, where Eulerian-mean flow
                   prognostic variables are solved for. Using the TWA
                   framework as a starting point, we explore the well
                   known connections between vertical transfer of
                   horizontal momentum by eddy form drag and eddy
                   overturning by the bolus velocity, used by Greatbatch
                   and Lamb (1990) and Gent and McWilliams (1990) (GM)
                   to parameterize eddies. After implementing the TWA
                   framework in an ocean general circulation model, we
                   verify our analysis by comparing the flows in an
                   idealized Southern Ocean configuration simulated
                   using the TWA and conventional frameworks with the
                   same meso-scale eddy parameterization.},
  annote =        {doi: 10.1175/JPO-D-15-0024.1},
  doi =           {10.1175/JPO-D-15-0024.1},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/JPO-D-15-0024.1},
}

@article{greatbatch_lamb_1990,
  author =        {Greatbatch, Richard J. and Lamb, Kevin G.},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2014/10/28},
  number =        {10},
  pages =         {1634--1637},
  publisher =     {American Meteorological Society},
  title =         {On Parameterizing Vertical Mixing of Momentum in
                   Non-eddy Resolving Ocean Models},
  volume =        {20},
  year =          {1990},
  abstract =      {Abstract We investigate the consequence, at small
                   Ekman number, of adding vertical mixing of momentum
                   terms to the incompressible thermocline equations. We
                   find that choosing the vertical eddy viscosity, ? =
                   Af2/N2, where f is the Coriolis parameter and N is
                   the local value of the buoyancy frequency, leads to
                   isopycnal mixing of fQ, where Q is the reciprocal of
                   potential vorticity, provided A is independent of the
                   vertical coordinate. If, additionally, A is also
                   independent of the north?south coordinate, then on a
                   beta-plane, this implies homogenization of potential
                   vorticity, q, within closed q-contours on isopycnal
                   surfaces. This conclusion extends to spherical
                   geometry if ? is also inversely proportional to ?,
                   the gradient of f with respect to latitude, i.e. ? =
                   Af2/(N2?). The connection with the recent work of
                   Gent and McWilliams and the consequences for coarse
                   resolution numerical model studies are discussed.},
  annote =        {doi: 10.1175/1520-0485(1990)020<1634:OPVMOM>2.0.CO;2},
  doi =           {10.1175/1520-0485(1990)020<1634:OPVMOM>2.0.CO;2},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/1520-0485(1990)020<1634:
                  OPVMOM>2.0.CO;2},
}

@article{ferrari_nikurashin_2010,
  author =        {Ferrari, Raffaele and Nikurashin, Maxim},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2015/03/11},
  number =        {7},
  pages =         {1501--1519},
  publisher =     {American Meteorological Society},
  title =         {Suppression of Eddy Diffusivity across Jets in the
                   Southern Ocean},
  volume =        {40},
  year =          {2010},
  abstract =      {Abstract Geostrophic eddies control the meridional
                   mixing of heat, carbon, and other climatically
                   important tracers in the Southern Ocean. The rate of
                   eddy mixing is typically quantified through an eddy
                   diffusivity. There is an ongoing debate as to whether
                   eddy mixing in enhanced in the core of the Antarctic
                   Circumpolar Current or on its flanks. A simple
                   expression is derived that predicts the rate of eddy
                   mixing, that is, the eddy diffusivity, as a function
                   of eddy and mean current statistics. This novel
                   expression predicts suppression of the cross-jet eddy
                   diffusivity in the core of the Antarctic Circumpolar
                   Current, despite enhanced values of eddy kinetic
                   energy. The expression is qualitatively and
                   quantitatively validated by independent estimates of
                   eddy mixing from altimetry observations. This work
                   suggests that the meridional eddy diffusivity across
                   the Antarctic Circumpolar Current is weaker than
                   presently assumed because of the suppression of eddy
                   mixing by the strong zonal current.},
  annote =        {doi: 10.1175/2010JPO4278.1},
  doi =           {10.1175/2010JPO4278.1},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/2010JPO4278.1},
}

@article{smith_2007,
  author =        {Smith, K. Shafer},
  journal =       {Journal of Marine Research},
  number =        {5},
  pages =         {655-683},
  title =         {The geography of linear baroclinic instability in
                   Earth's oceans},
  volume =        {65},
  year =          {2007},
  doi =           {doi:10.1357/002224007783649484},
}

@article{smith_marshall_2009,
  author =        {Smith, K. Shafer and Marshall, John},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2015/05/27},
  number =        {1},
  pages =         {50--69},
  publisher =     {American Meteorological Society},
  title =         {Evidence for Enhanced Eddy Mixing at Middepth in the
                   Southern Ocean},
  volume =        {39},
  year =          {2009},
  abstract =      {Abstract Satellite altimetric observations of the
                   ocean reveal surface pressure patterns in the core of
                   the Antarctic Circumpolar Current (ACC) that
                   propagate downstream (eastward) but slower than the
                   mean surface current by about 25{\%}. The authors
                   argue that these observations are suggestive of
                   baroclinically unstable waves that have a steering
                   level at a depth of about 1 km. Detailed linear
                   stability calculations using a hydrographic atlas
                   indeed reveal a steering level in the ACC near the
                   depth implied by the altimetric observations.
                   Calculations using a nonlinear model forced by the
                   mean shear and stratification observed close to the
                   core of the ACC, coinciding with a position where
                   mooring data and direct eddy flux measurements are
                   available, reveal a similar picture, albeit with
                   added details. When eddy fluxes are allowed to adjust
                   the mean state, computed eddy kinetic energy and eddy
                   stress are close to observed magnitudes with steering
                   levels between 1 and 1.5 km, broadly consistent with
                   observations. An important result of this study is
                   that the vertical structure of the potential
                   vorticity (PV) eddy diffusivity is strongly depth
                   dependent, implying that the diffusivity for PV and
                   buoyancy are very different from one another. It is
                   shown that the flow can simultaneously support a PV
                   diffusivity peaking at 5000 m2 s?1 or so near the
                   middepth steering level and a buoyancy diffusivity
                   that is much smaller, of order 1000 m2 s?1,
                   exhibiting less vertical structure. An effective
                   diffusivity calculation, using an advected and
                   diffused tracer transformed into area coordinates,
                   confirms that the PV diffusivity more closely
                   reflects the mixing properties of the flow than does
                   the buoyancy diffusivity, and points explicitly to
                   the need for separating tracer and buoyancy flux
                   parameterizations in coarse-resolution general
                   circulation models. Finally, implications for the
                   eddy-driven circulation of the ACC are discussed.},
  annote =        {doi: 10.1175/2008JPO3880.1},
  doi =           {10.1175/2008JPO3880.1},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/2008JPO3880.1},
}

@article{bates_etal_2014,
  author =        {Bates, Michael and Tulloch, Ross and Marshall, John and
                   Ferrari, Raffaele},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2015/03/12},
  number =        {6},
  pages =         {1523--1540},
  publisher =     {American Meteorological Society},
  title =         {Rationalizing the Spatial Distribution of Mesoscale
                   Eddy Diffusivity in Terms of Mixing Length Theory},
  volume =        {44},
  year =          {2014},
  abstract =      {AbstractObservations and theory suggest that lateral
                   mixing by mesoscale ocean eddies only reaches its
                   maximum potential at steering levels, surfaces at
                   which the propagation speed of eddies approaches that
                   of the mean flow. Away from steering levels, mixing
                   is strongly suppressed because the mixing length is
                   smaller than the eddy scale, thus reducing the mixing
                   rates. The suppression is particularly pronounced in
                   strong currents where mesoscale eddies are most
                   energetic. Here, a framework for parameterizing eddy
                   mixing is explored that attempts to capture this
                   suppression. An expression of the surface eddy
                   diffusivity proposed by Ferrari and Nikurashin is
                   evaluated using observations of eddy kinetic energy,
                   eddy scale, and eddy propagation speed. The resulting
                   global maps of eddy diffusivity have a broad
                   correspondence with recent estimates of diffusivity
                   based on the rate at which tracer contours are
                   stretched by altimetric-derived surface currents.
                   Finally, the expression for the eddy diffusivity is
                   extrapolated in the vertical to infer the
                   eddy-induced meridional heat transport and the
                   overturning streamfunction.},
  annote =        {doi: 10.1175/JPO-D-13-0130.1},
  doi =           {10.1175/JPO-D-13-0130.1},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/JPO-D-13-0130.1},
}

@book{smith_book_1997,
  author =        {Smith, Steven W and others},
  editor =        {California Technical Pub. San Diego},
  title =         {The scientist and engineer's guide to digital signal
                   processing},
  year =          {1997},
}

@article{chelton_etal_1998,
  author =        {Chelton, Dudley B. and deSzoeke, Roland A. and
                   Schlax, Michael G. and El Naggar, Karim and
                   Siwertz, Nicolas},
  booktitle =     {Journal of Physical Oceanography},
  journal =       {Journal of Physical Oceanography},
  month =         {2015/05/27},
  number =        {3},
  pages =         {433--460},
  publisher =     {American Meteorological Society},
  title =         {Geographical Variability of the First Baroclinic
                   Rossby Radius of Deformation},
  volume =        {28},
  year =          {1998},
  abstract =      {Abstract Global 1$\,^{\circ}$?
                   1$\,^{\circ}$climatologies of the first baroclinic
                   gravity-wave phase speed c1 and the Rossby radius of
                   deformation ?1 are computed from climatological
                   average temperature and salinity profiles. These new
                   atlases are compared with previously published
                   5$\,^{\circ}$? 5$\,^{\circ}$coarse resolution maps of
                   ?1 for the Northern Hemisphere and the South Atlantic
                   and with a 1$\,^{\circ}$?
                   1$\,^{\circ}$fine-resolution map of c1 for the
                   tropical Pacific. It is concluded that the methods
                   used in these earlier estimates yield values that are
                   biased systematically low by 5{\%}?15{\%} owing to
                   seemingly minor computational errors. Geographical
                   variations in the new high-resolution maps of c1 and
                   ?1 are discussed in terms of a WKB approximation that
                   elucidates the effects of earth rotation,
                   stratification, and water depth on these quantities.
                   It is shown that the effects of temporal variations
                   of the stratification can be neglected in the
                   estimation of c1 and ?1 at any particular location in
                   the World Ocean. This is rationalized from
                   consideration of the WKB approximation.},
  annote =        {doi: 10.1175/1520-0485(1998)028<0433:GVOTFB>2.0.CO;2},
  doi =           {10.1175/1520-0485(1998)028<0433:GVOTFB>2.0.CO;2},
  isbn =          {0022-3670},
  url =           {http://dx.doi.org/10.1175/1520-0485(1998)028<0433:
                  GVOTFB>2.0.CO;2},
}

@article{ringler_etal_2013,
  author =        {Todd Ringler and Mark Petersen and Robert L. Higdon and
                   Doug Jacobsen and Philip W. Jones and Mathew Maltrud},
  journal =       {Ocean Modelling},
  number =        {0},
  pages =         {211 - 232},
  title =         {A multi-resolution approach to global ocean modeling},
  volume =        {69},
  year =          {2013},
  doi =           {10.1016/j.ocemod.2013.04.010},
  issn =          {1463-5003},
  url =           {http://www.sciencedirect.com/science/article/pii/
                  S1463500313000760},
}

@article{thuburn_etal_2009,
  author =        {J. Thuburn and T.D. Ringler and W.C. Skamarock and
                   J.B. Klemp},
  journal =       {Journal of Computational Physics},
  number =        {22},
  pages =         {8321 - 8335},
  title =         {Numerical representation of geostrophic modes on
                   arbitrarily structured C-grids},
  volume =        {228},
  year =          {2009},
  abstract =      {A C-grid staggering, in which the mass variable is
                   stored at cell centers and the normal velocity
                   component is stored at cell faces (or edges in two
                   dimensions) is attractive for atmospheric modeling
                   since it enables a relatively accurate representation
                   of fast wave modes. However, the discretization of
                   the Coriolis terms is non-trivial. For constant
                   Coriolis parameter, the linearized shallow water
                   equations support geostrophic modes: stationary
                   solutions in geostrophic balance. A naive
                   discretization of the Coriolis terms can cause
                   geostrophic modes to become non-stationary, causing
                   unphysical behaviour of numerical solutions. Recent
                   work has shown how to discretize the Coriolis terms
                   on a planar regular hexagonal grid to ensure that
                   geostrophic modes are stationary while the Coriolis
                   terms remain energy conserving. In this paper this
                   result is extended to arbitrarily structured C-grids.
                   An explicit formula is given for constructing an
                   appropriate discretization of the Coriolis terms. The
                   general formula is illustrated by showing that it
                   recovers previously known results for the planar
                   regular hexagonal C-grid and the spherical
                   longitude--latitude C-grid. Numerical calculation
                   confirms that the scheme does indeed give stationary
                   geostrophic modes for the hexagonal--pentagonal and
                   triangular geodesic C-grids on the sphere.},
  doi =           {http://dx.doi.org/10.1016/j.jcp.2009.08.006},
  issn =          {0021-9991},
  url =           {http://www.sciencedirect.com/science/article/pii/
                  S0021999109004434},
}

@article{ringler_etal_2010,
  author =        {T.D. Ringler and J. Thuburn and J.B. Klemp and
                   W.C. Skamarock},
  journal =       {Journal of Computational Physics},
  number =        {9},
  pages =         {3065 - 3090},
  title =         {A unified approach to energy conservation and
                   potential vorticity dynamics for
                   arbitrarily-structured C-grids},
  volume =        {229},
  year =          {2010},
  doi =           {http://dx.doi.org/10.1016/j.jcp.2009.12.007},
  issn =          {0021-9991},
  url =           {http://www.sciencedirect.com/science/article/pii/
                  S0021999109006780},
}

@article{petersen_etal_2014,
  author =        {Mark R. Petersen and Douglas W. Jacobsen and
                   Todd D. Ringler and Matthew W. Hecht and
                   Mathew E. Maltrud},
  journal =       {Ocean Modelling},
  number =        {0},
  pages =         {93 - 113},
  title =         {Evaluation of the arbitrary Lagrangian--Eulerian
                   vertical coordinate method in the MPAS-Ocean model},
  volume =        {86},
  year =          {2015},
  doi =           {http://dx.doi.org/10.1016/j.ocemod.2014.12.004},
  issn =          {1463-5003},
  url =           {http://www.sciencedirect.com/science/article/pii/
                  S1463500314001796},
}

@article{skamarock_gassmann_2011,
  author =        {Skamarock, William C. and Gassmann, Almut},
  booktitle =     {Monthly Weather Review},
  journal =       {Monthly Weather Review},
  month =         {2014/12/11},
  number =        {9},
  pages =         {2962--2975},
  publisher =     {American Meteorological Society},
  title =         {Conservative Transport Schemes for Spherical Geodesic
                   Grids: High-Order Flux Operators for ODE-Based Time
                   Integration},
  volume =        {139},
  year =          {2011},
  abstract =      {AbstractHigher-order finite-volume flux operators for
                   transport algorithms used within Runge?Kutta time
                   integration schemes on irregular Voronoi (hexagonal)
                   meshes are proposed and tested. These operators are
                   generalizations of third- and fourth-order operators
                   currently used in atmospheric models employing
                   regular, orthogonal rectangular meshes.
                   Two-dimensional least squares fit polynomials are
                   used to evaluate the higher-order spatial derivatives
                   needed to cancel the leading-order truncation error
                   terms of the standard second-order centered
                   formulation. Positive definite or monotonic behavior
                   is achieved by applying an appropriate limiter during
                   the final Runge?Kutta stage within a given time
                   step.The third- and fourth-order formulations are
                   evaluated using standard transport tests on the
                   sphere. The new schemes are more accurate and
                   significantly more efficient than the standard
                   second-order scheme and other schemes in the
                   literature examined by the authors. The third-order
                   formulation is equivalent to the fourth-order
                   formulation plus an additional diffusion term that is
                   proportional to the Courant number. An optimal value
                   for the coefficient scaling this diffusion term is
                   chosen based on qualitative evaluation of the test
                   results. Improvements using the higher-order scheme
                   in place of the traditional second-order centered
                   approach are illustrated within 3D unstable
                   baroclinic wave simulations produced using two global
                   nonhydrostatic models employing spherical Voronoi
                   meshes.},
  annote =        {doi: 10.1175/MWR-D-10-05056.1},
  doi =           {10.1175/MWR-D-10-05056.1},
  isbn =          {0027-0644},
  url =           {http://dx.doi.org/10.1175/MWR-D-10-05056.1},
}

@article{ringler_etal_2017,
  author =        {Todd Ringler and Juan A. Saenz and Phillip J. Wolfram and
                   Luke Van Roekel},
  journal =       {Journal of Physical Oceanography},
  number =        {2},
  pages =         {285-302},
  title =         {A Thickness-Weighted Average Perspective of Force
                   Balance in an Idealized Circumpolar Current},
  volume =        {47},
  year =          {2017},
  abstract =      {AbstractThe exact, three-dimensional,
                   thickness-weighted averaged (TWA) Boussinesq
                   equations are used to diagnose eddy--mean flow
                   interaction in an idealized circumpolar current
                   (ICC). The force exerted by mesoscale eddies on the
                   TWA velocity is expressed as the divergence of the
                   Eliassen--Palm flux tensor. Consistent with previous
                   findings, the analysis indicates that the dynamically
                   relevant definition of the ocean surface layer is
                   composed of the set of buoyancy coordinates that ever
                   reside at the ocean surface at a given horizontal
                   position. The surface layer is found to be a
                   physically distinct object with a diabatic and force
                   balance that is largely isolated from the underlying
                   adiabatic region in the interior. Within the ICC
                   surface layer, the TWA meridional velocity is
                   southward/northward in the top/bottom half and has a
                   value near zero at the bottom. In the top half of the
                   surface layer, the zonal forces due to wind stress
                   and meridional advection of potential vorticity act
                   to accelerate the TWA zonal velocity; equilibrium is
                   obtained by eddies decelerating the zonal flow via a
                   downward flux of eastward momentum that increases
                   with depth. In the bottom half of the surface layer,
                   the accelerating force of the wind stress is balanced
                   by the eddy force and meridional advection of
                   potential vorticity. The bottom of the surface layer
                   coincides with the location where the zonal eddy
                   force, meridional advection of potential vorticity,
                   and zonal wind stress force are all zero. The net
                   meridional transport Sf within the surface layer is a
                   small residual of its southward and northward TWA
                   meridional flows. The mean meridional gradient of the
                   surface layer buoyancy is advected by Sf to balance
                   the surface buoyancy flux.},
  doi =           {10.1175/JPO-D-16-0096.1},
  url =           {http://dx.doi.org/10.1175/JPO-D-16-0096.1},
}

@article{large_etal_1994,
  author =        {Large, W. G. and McWilliams, J. C. and Doney, S. C.},
  journal =       {Rev. Geophys.},
  number =        {4},
  pages =         {363--403},
  publisher =     {AGU},
  title =         {Oceanic vertical mixing: A review and a model with a
                   nonlocal boundary layer parameterization},
  volume =        {32},
  year =          {1994},
  abstract =      {If model parameterizations of unresolved physics,
                   such as the variety of upper ocean mixing processes,
                   are to hold over the large range of time and space
                   scales of importance to climate, they must be
                   strongly physically based. Observations, theories,
                   and models of oceanic vertical mixing are surveyed.
                   Two distinct regimes are identified: ocean mixing in
                   the boundary layer near the surface under a variety
                   of surface forcing conditions (stabilizing,
                   destabilizing, and wind driven), and mixing in the
                   ocean interior due to internal waves, shear
                   instability, and double diffusion (arising from the
                   different molecular diffusion rates of heat and
                   salt). Mixing schemes commonly applied to the upper
                   ocean are shown not to contain some potentially
                   important boundary layer physics. Therefore a new
                   parameterization of oceanic boundary layer mixing is
                   developed to accommodate some of this physics. It
                   includes a scheme for determining the boundary layer
                   depth h, where the turbulent contribution to the
                   vertical shear of a bulk Richardson number is
                   parameterized. Expressions for diffusivity and
                   nonlocal transport throughout the boundary layer are
                   given. The diffusivity is formulated to agree with
                   similarity theory of turbulence in the surface layer
                   and is subject to the conditions that both it and its
                   vertical gradient match the interior values at h.
                   This nonlocal \&{\#}8220;K profile
                   parameterization\&{\#}8221; (KPP) is then verified
                   and compared to alternatives, including its
                   atmospheric counterparts. Its most important feature
                   is shown to be the capability of the boundary layer
                   to penetrate well into a stable thermocline in both
                   convective and wind-driven situations. The
                   diffusivities of the aforementioned three interior
                   mixing processes are modeled as constants, functions
                   of a gradient Richardson number (a measure of the
                   relative importance of stratification to
                   destabilizing shear), and functions of the
                   double-diffusion density ratio, R\&{\#}961;. Oceanic
                   simulations of convective penetration, wind
                   deepening, and diurnal cycling are used to determine
                   appropriate values for various model parameters as
                   weak functions of vertical resolution. Annual cycle
                   simulations at ocean weather station Papa for 1961
                   and 1969\&{\#}8211;1974 are used to test the complete
                   suite of parameterizations. Model and observed
                   temperatures at all depths are shown to agree very
                   well into September, after which systematic advective
                   cooling in the ocean produces expected differences.
                   It is argued that this cooling and a steady salt
                   advection into the model are needed to balance the
                   net annual surface heating and freshwater input. With
                   these advections, good multiyear simulations of
                   temperature and salinity can be achieved. These
                   results and KPP simulations of the diurnal cycle at
                   the Long-Term Upper Ocean Study (LOTUS) site are
                   compared with the results of other models. It is
                   demonstrated that the KPP model exchanges properties
                   between the mixed layer and thermocline in a manner
                   consistent with observations, and at least as well or
                   better than alternatives.},
  isbn =          {8755-1209},
  url =           {http://dx.doi.org/10.1029/94RG01872},
}


